DeepSITH: Efficient Learning via Decomposition of What and When Across Time Scales

Extracting temporal relationships over a range of scales is a hallmark of human perception and cognition -- and thus it is a critical feature of machine learning applied to real-world problems. Neural networks are either plagued by the exploding/vanishing gradient problem in recurrent neural networks (RNNs) or must adjust their parameters to learn the relevant time scales (e.g., in LSTMs). This paper introduces DeepSITH, a network comprising biologically-inspired Scale-Invariant Temporal History (SITH) modules in series with dense connections between layers. SITH modules respond to their inputs with a geometrically-spaced set of time constants, enabling the DeepSITH network to learn problems along a continuum of time-scales. We compare DeepSITH to LSTMs and other recent RNNs on several time series prediction and decoding tasks. DeepSITH achieves state-of-the-art performance on these problems.

==> NeurIPS DeepSITH_arxiv/checklist <==
checklist:


- check N_i should be used in 1.3
- check lowercase k in table
- check tau \ prediction distance
- add lindeberg and fagerstrom citation, and lindeberg and janssen, and smith and sommer 2013
- Give section PARAMETERIZATIONS OF DEEPSITH a reread. 


==> checklist <==
checklist:


- check N_i should be used in 1.3
- check lowercase k in table
- check tau \ prediction distance
- add lindeberg and fagerstrom citation, and lindeberg and janssen, and smith and sommer 2013
- Give section PARAMETERIZATIONS OF DEEPSITH a reread. 

